V-Fuzz: Vulnerability-Oriented Evolutionary Fuzzing

Fuzzing is a technique of finding bugs by executing a software recurrently with a large number of abnormal inputs. Most of the existing fuzzers consider all parts of a software equally, and pay too much attention on how to improve the code coverage. It is inefficient as the vulnerable code only takes a tiny fraction of the entire code. In this paper, we design and implement a vulnerability-oriented evolutionary fuzzing prototype named V-Fuzz, which aims to find bugs efficiently and quickly in a limited time. V-Fuzz consists of two main components: a neural network-based vulnerability prediction model and a vulnerability-oriented evolutionary fuzzer. Given a binary program to V-Fuzz, the vulnerability prediction model will give a prior estimation on which parts of the software are more likely to be vulnerable. Then, the fuzzer leverages an evolutionary algorithm to generate inputs which tend to arrive at the vulnerable locations, guided by the vulnerability prediction result. Experimental results demonstrate that V-Fuzz can find bugs more efficiently than state-of-the-art fuzzers. Moreover, V-Fuzz has discovered 10 CVEs, and 3 of them are newly discovered. We reported the new CVEs, and they have been confirmed and fixed.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> abstract.tex <==
Fuzzing is a technique of finding bugs by executing a software recurrently with a large number of abnormal inputs.\\
Most of the existing fuzzers consider all parts of a software equally,
and pay too much attention on how to improve the code coverage.
It is inefficient as the vulnerable code only takes a tiny fraction of the entire code.
In this paper, 
we design and implement a vulnerability-oriented evolutionary fuzzing prototype named V-Fuzz, 
which aims to find bugs efficiently and quickly in a limited time.
V-Fuzz consists of two main components:  
a \emph{neural network-based vulnerability prediction model}
and a \emph{vulnerability-oriented evolutionary fuzzer}. 
Given a binary program to V-Fuzz, 
the vulnerability prediction model will give a prior estimation on which parts of the software are more likely to be vulnerable.
Then,
the fuzzer leverages an evolutionary algorithm to generate inputs which tend to arrive at the vulnerable locations,  
guided by the vulnerability prediction result. 
% We implement V-Fuzz and evaluate it with 10 real-world Linux applications 
% and three popular fuzzing benchmark programs of LAVA-M.
Experimental results demonstrate that V-Fuzz can find bugs more efficiently than state-of-the-art fuzzers.
Moreover,
V-Fuzz has discovered 10 CVEs, 
and 3 of them are newly discovered.\\
We reported the new CVEs, 
and they have been confirmed and fixed.

==> ref-temp.tex <==
--------------------------------------

\bibitem{Shin2011Evaluating}
Y. Shin, A. Meneely, L. Williams, and J. A. Osborne,
``Evaluating complexity code chrun, and developer activity metrics as indicators of software vulnerabilities,''
\emph{IEEE Transactions on Software Engineering},
2011, 
37(6): 772-787.

\bibitem{Hovsepyan2012Software}
A. Hovsepyan, R. Scandariato, W. Joosen, and J. Walden, 
``Software vulnerability prediction using text analysis techniques,''
\emph{Proceedings of the 4th international workshop on Security measurements and metrics},
ACM, 2012: 7-10.

\bibitem{Gegick2008Prioritizing}
M. Gegick, L. Williams, J. Osborne, and M. Vouk, 
``Prioritizing software security fortification through code-level metrics,''
\emph{Proceedings of the 4th ACM workshop on Quality of protection},
ACM, 2008: 31-38.

\bibitem{Neuhaus2007Predicting}
S. Neuhaus, T. Zimmermann, C. Holler, and A. Zeller，
``Predicting vulnerable software components,''
\emph{Proceedings of the 14th ACM conference on Computer and communications security},
ACM, 2007: 529-540.

\bibitme{Shar2013Mining}
L. K. Shar, H. B. K. Tan, and L. C. Briand,
``Mining SQL injection and cross site scripting vulnerabilities using hybrid program analysis,''
\emph{Proceedings of the 2013 International Conference on Software Engineering},
IEEE Press, 2013: 642-651.

% \bibitme{Shar2012Predicting}
% L. K. Shar and H. B. K. Tan,
% ``Predicting common web application vulnerabilities from input validation and sanitization code patterns'',
% \emph{Proceedings of the 27th IEEE/ACM International Conference on Automated Software Engineering (ASE)},
%  IEEE, 2012: 310-313.


% \bibitme{47}
%  B. Smith and L. Williams,
%  ``Using SQL hotspots in a prioritization heuristic for detecting all types of web application vulnerabilities,''
%  \emph{Proceedings of the 4th International Conference on Software Testing, Verification and Validation (ICST)},
% IEEE, 2011: 220-229.

% Walden J, Doyle M, Welch G A, et al. [C]//, 2009. ESEM 2009. 3rd International Symposium on. 

% \bibitme{48}
%  J. Walden, M. Doyle, G. A. Welch, and M. Whelan,
%  ``Security of open source web applications,''
%  \emph{Proceedings of the 3rd International Symposium on Empirical Software Engineering and Measurement}
% IEEE, 2009: 545-553.


% Walden J, Stuckman J, Scandariato R. [C]//, 2014 IEEE 25th International Symposium on. 
% Walden, J., Stuckman, J., & Scandariato, R. (2014, November). Predicting vulnerable components: Software metrics vs text mining. In Software Reliability Engineering (ISSRE), 2014 IEEE 25th International Symposium on (pp. 23-33). IEEE.

\bibitme{10}
 J. Walden, J. Stuckman, and R. Scandariato,
 ``Predicting vulnerable components: Software metrics vs text mining,''
 \emph{Proceedings of the 25th International Symposium on Software Reliability Engineering (ISSRE)},
 IEEE, 2014: 23-33.





-------------------------------------------------------------------------------------------
% Dam, H. K., Tran, T., Pham, T., Ng, S. W., Grundy, J., & Ghose, A. (2017). Automatic feature learning for vulnerability prediction. 


\bibitem{Dam2017Automatic}
H. K. Dam, T. Tran, T. Pham et al. 
``Automatic feature learning for vulnerability prediction.''
\emph{arXiv preprint arXiv:1708.02368.},
2017


\bibitem{Wang2016Automatic}
S. Wang, T. Liu, and L. Tan,
``Automatically learning semantic features for defect prediction,''
\emph{Proceedings of the 38th International Conference on Software Engineering},
ACM, 2016, pp. 297–308.
% New York,
% NY, USA

\bibitem{Yang2015Deep} 
X. Yang, D. Lo, X. Xia, Y. Zhang, and J. Sun,
``Deep learning for just-in-time defect prediction,''
\emph{Proceedings of the 2015 IEEE International Conference on Software Quality, Reliability and Security},
IEEE Computer Society, 2015,
pp. 17–26.


\bibitem{Dam2016DeepSoft}
H. K. Dam, T. Tran, J. Grundy, and A. Ghose,
``DeepSoft: A vision for a deep model of software,''
\emph{Proceedings of the 24th ACM SIGSOFT International Symposium on Foundations of Software Engineering},
ACM, 2016.


\bibitem{White2015Toward}
M. White, C. Vendome, M. Linares-Vásquez, and D. Poshyvanyk,
``Toward deep learning software repositories,''
\emph{Proceedings of the 12th Working Conference on Mining Software Repositories},
IEEE Press, 2015, pp. 334–345.


\bibitem{Gu2016Deep}
X. Gu, H. Zhang, D. Zhang, and S. Kim,
``Deep api learning''
\emph{Proceedings of the 2016 24th ACM SIGSOFT International Symposium on Foundations of Software Engineering},
ACM, 2016, pp. 631–642.

\bibitem{Gupta2017Deepfix}
R. Gupta, S. Pal, A. Kanade, and S. Shevade,
``Deepfix: Fixing common C language errors by deep learning'',
\emph{Proceedings of the 31st AAAI Conference on Artificial Intelligence},
2017, pp. 1345–1351.

\bibitem{Huo2016Learning}
X. Huo, M. Li, and Z.-H. Zhou,
``Learning unified features from natural and programming languages for locating buggy source code'',
\emph{Proceedings of the 25th International Joint Conference on Artificial Intelligence},
 2016, pp. 1606–1612.

% \bibitem{Dam2016A}
% H. K. Dam, T. Tran, and T. Pham,
% ``A deep language model for software code,''
% \emph{Workshop on Naturalness of Software (NL+SE), co-
% located with the 24th ACM SIGSOFT International Symposium on the
% Foundations of Software Engineering (FSE)},
% 2016.

-------------------------------------------------------------------------------------------


==> related_work_VP.tex <==


There are 29 papers related to vulnerability prediction.



% \bibitem{bottinger2018deep}
% K.~B{\"o}ttinger, P.~Godefroid, and R.~Singh, "Deep reinforcement fuzzing,"
%   \emph{arXiv preprint arXiv:1801.04589}, 2018.

\bibitem{cai2018comprehensive}
H.~Cai, V.~Zheng, and K.~Chang, "A comprehensive survey of graph embedding:
  problems, techniques and applications," \emph{IEEE Transactions on Knowledge
  and Data Engineering}, 2018.


\bibitem{2018-zhe-yu} 
Z. Yu, C. Theisen, H. Sohn, L. Williams and T. Menzies,
``Cost-aware Vulnerability Prediction: the HARMLESS Approach'',
\emph{http://arxiv.org/abs/1803.06545},
2018.




